DPO Kernels: A Semantically-Aware, Kernel-Enhanced, and Divergence-Rich Paradigm for Direct Preference Optimization

The rapid rise of large language models (LLMs) has unlocked many applications but also underscores the challenge of aligning them with diverse values and preferences. Direct Preference Optimization (DPO) is central to alignment but constrained by fixed divergences and limited feature transformations. We propose DPO-Kernels, which integrates kernel methods to address these issues through four key contributions: (i) Kernelized Representations with polynomial, RBF, Mahalanobis, and spectral kernels for richer transformations, plus a hybrid loss combining embedding-based and probability-based objectives; (ii) Divergence Alternatives (Jensen-Shannon, Hellinger, Renyi, Bhattacharyya, Wasserstein, and f-divergences) for greater stability; (iii) Data-Driven Selection metrics that automatically choose the best kernel-divergence pair; and (iv) a Hierarchical Mixture of Kernels for both local precision and global modeling. Evaluations on 12 datasets demonstrate state-of-the-art performance in factuality, safety, reasoning, and instruction following. Grounded in Heavy-Tailed Self-Regularization, DPO-Kernels maintains robust generalization for LLMs, offering a comprehensive resource for further alignment research.

==> 2_axioms.tex <==


\begin{figure}[h!]
    \centering
    \includegraphics[width=\columnwidth]{img/alignment_axioms.png}
    \caption{\cite{} categorized human values into seven distinct groups: (i) information seeking, (ii) wisdom and knowledge, (iii) well-being and peace, (iv) justice and rights, (v) duty and accountability, (vi) civility and tolerance, and (vii) empathy and helpfulness}
    \label{fig:pentagon}
\end{figure}


\section{Axioms of Alignment}

In principle, alignment techniques should ensure that large language models (LLMs) reflect human-preferred values. However, very limited research has investigated which specific human values are operationalized within existing datasets. The pioneering study by \cite{obi2024valueimprinttechniqueauditing} addresses this gap by categorizing human values into seven distinct groups: (i) information seeking, (ii) wisdom and knowledge, (iii) well-being and peace, (iv) justice and rights, (v) duty and accountability, (vi) civility and tolerance, and (vii) empathy and helpfulness. These seven values are further organized into four broader categories: well-being and safety, information utility, civic values, and pro-social values, as depicted in Figure~\ref{fig:values_categorization}. The authors released an annotated dataset organized according to these seven classes.

Our research seeks to explore the following questions:

\textbf{RQ1}: Which human values are relatively complex for alignment methods?

\textbf{RQ2}: Is there a possibility that different combinations of RKD (Representations, Kernels, and Divergence) are suitable for different values?

\textbf{RQ3}: Is there a method that can generalize across various values?

\textbf{RQ4}: Do aligned models exhibit loss generalizability?

On one hand, we introduce foundational innovations based on RKD to enhance the DPO framework. On the other hand, we identify the most suitable kernel functions for specific value alignments. 


==> 4_eval.tex <==














\section{Assessing the Alignment of LLMs}

1. G-eval: https://arxiv.org/abs/2303.16634\\
2. Analyze-Rate: https://arxiv.org/abs/2310.05657\\
3. ReFeR: https://arxiv.org/abs/2407.12877\\
4. Reconcile: https://arxiv.org/abs/2309.13007


==> 6_layers.tex <==



\section{Aligned Layer in LLMs} 
\label{sec:performance}


Model-Oriented Sub-population and Spectral Analysis (MOSSA; Zhao et al. 2022) \\
Center Kernel Alignment (CKA; Kornblith et al., 2019)\\

\begin{figure}
    \centering
    \includegraphics[width=\columnwidth]{img/layer_by_layer.png}
    \caption{blah blah blah....}
    \label{fig:pentagon}
\end{figure}



\begin{tcolorbox}[
left=9pt,right=2pt,colback=Olive!5!white,colframe=Olive!75!black,colbacktitle=Olive,
  title=\footnotesize \fontfamily{qbk} \selectfont \textbf{Implications derived from $\mathbf{HVI_{auto}}$} ]
  
\vspace{-2mm}
\begin{itemize}
[labelindent=-0.2em,labelsep=0.1cm,leftmargin=*]
\setlength\itemsep{0em}
\begin{spacing}{0.85}

\item[\ding{118}] 
{\footnotesize 
{\fontfamily{phv}\fontsize{7}{8}
%\begin{spacing}{1}
\selectfont
Larger LLMs without RLHF \cite{DBLP:journals/corr/abs-1909-08593} are prone to hallucination, as shown in \cref{tab:hvi_spectrum}. 
}
%\end{spacing}
}
\vspace{-1mm} 
\item[\ding{118}] 
{\footnotesize 
{\fontfamily{phv}\fontsize{7}{8}
%\begin{spacing}{1}
\selectfont
Number-related issues are widespread across most LLMs, although they appear notably lower in certain models such as XLNet and StableLM. The reasons behind this discrepancy remain unclear and warrant further investigation in the future.}
%\end{spacing}
}
\vspace{-1mm} 
\item[\ding{118}] 
{\footnotesize 
{\fontfamily{phv}\fontsize{7}{8}
%\begin{spacing}{1}
\selectfont
Hallucination categories such as Imaginary Figures and Temporal issues tend to increase with the size of LLMs.
}
%\end{spacing}
}
%\end{spacing}

\vspace{-6mm}
\end{spacing}
\end{itemize}
\end{tcolorbox}





==> 7_generalization.tex <==
\section{Assessing Generalization \& Model Quality}  
\label{sec:auto-hvi}

Frobenius Norm\\
Spectral Norm\\
Weighted Alpha\\



\begin{figure}
    \centering
    \includegraphics[width=0.6\columnwidth]{img/overlay.png}
    \caption{blah blah blah....}
    \label{fig:pentagon}
\end{figure}







\begin{tcolorbox}[
left=9pt,right=2pt,colback=Olive!5!white,colframe=Olive!75!black,colbacktitle=Olive,
  title=\footnotesize \fontfamily{qbk} \selectfont \textbf{Implications derived from $\mathbf{HVI_{auto}}$} ]
  
\vspace{-2mm}
\begin{itemize}
[labelindent=-0.2em,labelsep=0.1cm,leftmargin=*]
\setlength\itemsep{0em}
\begin{spacing}{0.85}

\item[\ding{118}] 
{\footnotesize 
{\fontfamily{phv}\fontsize{7}{8}
%\begin{spacing}{1}
\selectfont
Larger LLMs without RLHF \cite{DBLP:journals/corr/abs-1909-08593} are prone to hallucination, as shown in \cref{tab:hvi_spectrum}. 
}
%\end{spacing}
}
\vspace{-1mm} 
\item[\ding{118}] 
{\footnotesize 
{\fontfamily{phv}\fontsize{7}{8}
%\begin{spacing}{1}
\selectfont
Number-related issues are widespread across most LLMs, although they appear notably lower in certain models such as XLNet and StableLM. The reasons behind this discrepancy remain unclear and warrant further investigation in the future.}
%\end{spacing}
}
\vspace{-1mm} 
\item[\ding{118}] 
{\footnotesize 
{\fontfamily{phv}\fontsize{7}{8}
%\begin{spacing}{1}
\selectfont
Hallucination categories such as Imaginary Figures and Temporal issues tend to increase with the size of LLMs.
}
%\end{spacing}
}
%\end{spacing}

\vspace{-6mm}
\end{spacing}
\end{itemize}
\end{tcolorbox}


